Communication Lower Bounds for Statistical Estimation Problems via a Distributed Data Processing Inequality

We study the tradeoff between the statistical error and communication cost of distributed statistical estimation problems in high dimensions. In the distributed sparse Gaussian mean estimation problem, each of the $m$ machines receives $n$ data points from a $d$-dimensional Gaussian distribution with unknown mean $\theta$ which is promised to be $k$-sparse. The machines communicate by message passing and aim to estimate the mean $\theta$. We provide a tight (up to logarithmic factors) tradeoff between the estimation error and the number of bits communicated between the machines. This directly leads to a lower bound for the distributed \textit{sparse linear regression} problem: to achieve the statistical minimax error, the total communication is at least $\Omega(\min\{n,d\}m)$, where $n$ is the number of observations that each machine receives and $d$ is the ambient dimension. These lower results improve upon [Sha14,SD'14] by allowing multi-round iterative communication model. We also give the first optimal simultaneous protocol in the dense case for mean estimation. As our main technique, we prove a \textit{distributed data processing inequality}, as a generalization of usual data processing inequalities, which might be of independent interest and useful for other problems.

==> main_theory.tex <==
\section{Distributed Strong Data Processing Inequalities}\label{sec:main-theorem}
In this section we prove our main Theorem~\ref{thm:main-intro}. We state a slightly weaker looking version here but in fact it implies Theorem~\ref{thm:main-intro} by symmetry. The same proof also goes through for the case when the RHS is conditioned on $V=1$.

\begin{theorem}\label{thm:main-asymmetric}
	Suppose $\mu_1\le c\cdot \mu_0$, and $\beta(\mu_0,\mu_1) = \beta$, we have %Suppose $\mu_1\le O(1)\cdot\mathcal{D}_0$ and $(\mu_0,\mu_1)$ satisfies the data processing inequality (\ref{eqn:data_processing}) for parameter $\beta$, 
	%then for $X\sim \mathcal{D}_{\bs{0}}$ we have 
	\begin{equation}
	\h^2(\Pi\vert_{V=0}, \Pi\vert_{V=1}) \le O(1)\cdot \frac{(c+1)\beta}{2}\cdot\I(X;\Pi\mid V=0) \,.\label{eqn:sdpi-main-theorem}
	\end{equation}
\end{theorem}

\noindent Note that the RHS of~\eqref{eqn:sdpi-main-theorem} naturally tensorizes in the sense that 
\begin{equation}
\sum_{i=1}^m \I(X_i;\Pi\mid V=0)\le \I(X;\Pi\mid V=0),\label{eqn:dsdpi-inter6}
\end{equation}

since conditioned on $V = 0$, the $X_i$'s are independent with each other. Our main idea consists of the following two steps a) We will tensorize the LHS of~\eqref{eqn:sdpi-main-theorem} so that the target inequality~\eqref{eqn:sdpi-main-theorem} can be written as a sum of $m$ inequalities. b) We prove each of these $m$ inequalities using the single machine SDPI. 
%In this section 



%\Tnote{Note below $V,X,\Pi$ have a special joint distribution. Though we use the same letters. }
To this end, we do the following thought experiment: Suppose $W$ is a random variable that takes value from $\{0,1\}$ uniformly. Suppose data $X'$ is generated as follows: $X'_j\sim \mu_W$, and for any $j\neq i$, $X_j' \sim \mu_0$. We apply the protocol on the input $X'$, and view the resulting transcript $\Pi'$ as communication between $i$-th machine and the remaining machines. Then we are in the situation of a single machine case, that is, $W\rightarrow X_i'\rightarrow \Pi'$ forms a Markov Chain. Applying the data processing inequality~\eqref{eqn:data-processing-inequality-intro}, we obtain that 
\begin{equation}
\I(W';\Pi')\le \beta \I(X_i';\Pi') \cdot \label{eqn:dsdpi-inter8}
\end{equation}
Using Lemma~\ref{lem:info-hellinger}, we can lower bound the LHS of~\eqref{eqn:dsdpi-inter8} by the Hellinger distance and obtain
\begin{equation}
\h^2(\Pi'\vert_{W=0}, \Pi'\vert_{W=1})\le \beta \cdot\I(X_i';\Pi') \nonumber %\label{eqn:dsdpi-inter11}
\end{equation}
Let $\bs{e_i} = (0,0,\dots,1,\dots,0)$ be the unit vector that only takes 1 in the $i$th entry, and $\bs{0}$ the all zero vector. Using the notation defined in Section~\ref{subsec:cut-paste}, we observe that $\Pi'\vert_{W=0}$ has distribution $\Pi_{\bs{0}}$ while  $\Pi'\vert_{W=1}$ has distribution $\Pi_{\bs{e}_i}$. Then we can rewrite the equation above as 
\begin{equation}
\h^2(\Pi_{\bs{0}}, \Pi_{\bs{e}_i})\le \beta \cdot\I(X_i';\Pi') \label{eqn:dsdpi-inter11}
\end{equation}
Observe that the RHS of~\eqref{eqn:dsdpi-inter11} is close to the first entry of the LHS of~\eqref{eqn:dsdpi-inter6} since the joint distribution of $(X_1',\Pi')$ is not very far from $X,\Pi\mid V=0$. (The only difference is that $X_1'$ is drawn from a mixture of $\mu_0$ and $\mu_1$, and note that $\mu_0$ is not too far from $\mu_1$). On the other hand, the sum of LHS of~\eqref{eqn:dsdpi-inter11} over $i\in [m]$ is lower-bounded by the LHS of~\eqref{eqn:sdpi-main-theorem}. Therefore, we can tensorize equation~\eqref{eqn:sdpi-main-theorem} into inequality~\eqref{eqn:dsdpi-inter11} which can be proved by the single machine SDPI.  %which can be viewed as a ternsorization of hellinger distance.
%To make this intuition formal, we use the notations.  
 %When $X\sim \mu_{\bs{0}}$,  assume that $\Pi$ doesn't release much information of $X_i$. Then by data processing inequality, intuitively if one replaces the data generating distribution $\mu_0$ by $\mu_1$ locally on machine $i$, then the distribution of $\Pi$ won't change a lot. We formalize this intuition by the following lemma. 
 We formalize the intuition above by the following two lemmas, 
\begin{lemma}\label{lem:mutual-info-hellinger}
	Suppose $\mu_1\le c\cdot\mu_0$, and $\beta(\mu_0,\mu_1) = \beta$,  then %and $(\mu_0,\mu_1)$ satisfies the data processing inequality (\ref{eqn:data_processing}) for parameter $\beta$, 
	%then for $X\sim \mathcal{\mu}_{\bs{0}}$ we have 
	\begin{equation}
		\h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}})\le \frac{(c+1)\beta}{2}\cdot \I(X_i;\Pi\mid V=0) 
	\end{equation}
%	\begin{equation}
%		\sum_{i=1}^m \I(X_i;\Pi) \ge\Omega(\beta^{-1}) \h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}})
%	\end{equation}
\end{lemma}

\begin{lemma}\label{lem:hellinger-decomposition}
	Let $\bs{0}$ be the $m$-dimensional all 0's vector, and $\bs{1}$ the all 1's vector, we have that 
	$$\h^2(\Pi_{\bs{0}},\Pi_{\bs{1}})\le O(1)\cdot\sum_{i=1}^m \h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}}) $$
\end{lemma}

Using Lemma~\ref{lem:mutual-info-hellinger} and Lemma~\ref{lem:hellinger-decomposition}, we obtain Theorem~\ref{thm:main-asymmetric} straightforwardly

\begin{proof}[Proof of Theorem~\ref{thm:main-asymmetric}]
	First by Lemma~\ref{lem:mutual-info-additivity}, we can decompose $\I(X;\Pi)$ by 
	$$  \sum_{i=1}^m \I(X_i;\Pi\mid V=0)\le \I(X;\Pi\mid V=0)\,. $$
	Then invoking Lemma~\ref{lem:mutual-info-hellinger}, we can lower bound $ \I(X_i;\Pi)$ by the Hellinger distance between $\Pi_{\bs{e_i}}$ and $\Pi_{\bs{0}}$. 
	\begin{equation*}
\h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}})\le \frac{(c+1)\beta}{2} \cdot	\I(X_i;\Pi\mid V=0)\,. 
	\end{equation*}
	Then by Lemma~\ref{lem:hellinger-decomposition}, we have
	$$\h^2(\Pi_{\bs{0}}, \Pi_{\bs{1}})\le O(1)\cdot\sum_{i=1}^{m} \h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}}) \,. $$
	Then the desired inequality follows by combining the inequalities above. 
\end{proof}
%\begin{remark}
%	It seems that the condition $\mu_1 \le O(1) \mu_0$ should be an artifact of our proof strategy, and not essential. However, we argue that this condition is fairly weak and does not hurt us much because in principle, when $\beta(\mu_0,\mu_1)\ll 1$, $\mu_0(x)\le O(1)\cdot \mu_0(x)$ should be true for most points $x$. % b) when $\mu_0(x)\le O(1)\cdot \mu_0(x)$ is not terribly wrong, usually the conclusion itself is not tight either and we can use other (e,g, the trivial) ways to lower bound $\I(X;\Pi)$. 
	%In principle, the condition $\mu_1 \le O(1) \mu_0$ should be dominated by the condition that $\beta(\mu_0,\mu_1)$ is small, in which case the result is strong and interesting. (In most of our cases, $\beta$ is on the order of $1/m$.) %For example, Duchi et al.~\cite{DBLP:journals/corr/DuchiJWZ14} roughly shows that if $(1-\alpha)\mu_1 \le \mu_0 \le (1+\alpha) \mu_1$, then $\beta(\mu_0,\mu_1)\le O(\alpha^2)$. 
%\end{remark}
%\begin{remark}
%	When we apply the theorem later for Gaussian distributions, we truncate the Gaussian distribution first on some interval $[-\tau,\tau]$ on which $\mu_0 \le O(1)\cdot \mu_1$ is true, and then argue that the probability mass outside $[-\tau,\tau]$ is too small to cause a difference. 
%\end{remark}
Finally we provide the proof of Lemma~\ref{lem:mutual-info-hellinger}. Lemma~\ref{lem:hellinger-decomposition} is a direct corollary of Theorem~\ref{thm:hellinger-sum} (which is in turn a direct corollary of Theorem 7 of~\cite{Hellinger}) and Proposition~\ref{prop:cut-paste}. 
\begin{proof}[Proof of Lemma~\ref{lem:mutual-info-hellinger}] %\Tnote{proof needs some revise}
 %Let $\bar{\mu}_i := \frac{1}{2}(\mu_{\bs{e_i}}+ \mu_{\bs{0}})$. 
 Let $W$ be uniform Bernoulli and define $X'$ and $\Pi'$ as follows: Conditioned on $W = 0$, $X'\sim \mu_{\bs{0}}$ and conditioned on $W = 1$, $X'\sim \mu_{\bs{e_i}}$. We run protocol on $X'$ and get transcript $\Pi'$. 
 
 Note that $V\rightarrow X' \rightarrow \Pi'$ is a Markov chain and so is $V\rightarrow X_i'\rightarrow \Pi'$. Also by definition, $P_{X'\mid V}$ is the same channel as in Definition~\ref{def:sdpi-intro}. Therefore by Definition~\ref{def:sdpi-intro}, we have that 
 
 %Consider the following joint distribution $\calP_i$ of $V,X', \Pi'$ defined as follows . Let $V$ be uniform random variable over $\{0,1\}$. Conditioned on $V =v$, we draw $X_i'$ from $\mu_v$. For all $j\neq i$, we draw $X_j'$ from $\mu_0$. Then we run the protocol on $X_1',\dots, X_m'$ and obtain $\Pi(X_1',\dots,X_m')$. Note that under this joint distribution, the marginal distribution of $(X_1',\dots,X_m')$ is actually $\bar{\mu}_i$, and $V, X_i', \Pi'$ forms a Markov Chain. The joint distribution of $V, X_i'$ is the same as described before equation (\ref{eqn:data_processing}). Therefore assuming equation (\ref{eqn:data_processing}) is true for some $\beta$, then 
\begin{equation}
\beta\cdot \I(X_i';\Pi') \ge \I(V;\Pi').\label{eqn:1}
\end{equation}
It is known that mutual information can be expressed as the expectation of KL divergence, which in turn is lower-bounded by Hellinger distance. We invoke a technical variant of this argument, Lemma 6.2 of~\cite{DBLP:journals/jcss/Bar-YossefJKS04}, restated as Lemma~\ref{lem:info-hellinger}, to lower bound the right hand side. Note that $Z$ in Lemma~\ref{lem:info-hellinger} corresponds to $V$ here and $\phi_{z_1},\phi_{z_2}$ corresponda to $\Pi_{\bs{e_i}}$ and $\Pi_{\bs{0}}$. Therefore, we conclude
\begin{equation}
	\I(V;\Pi') \ge \h ^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}}).\label{eqn:2}
\end{equation} 
It remains to relate $\I(X_i';\Pi')$ with $\I(X_i;\Pi\mid V=0)$. Note that the difference between joint distributions of $(X_i',\Pi')$ and $(X_i,\Pi)\vert_{V=0}$ is that $X_i'\sim \frac{1}{2}(\mu_0+\mu_1)$ and $X_i\vert_{V=0}\sim \mu_0$.  %where $X\sim \mu_{\bs{0}}$. 
We claim (by Lemma~\ref{lem:continuity}) that since $\mu_{0}\ge \frac{2}{c+1}(\frac{\mu_0+\mu_1}{2})$, we have 
\begin{equation}
	\I(X_i;\Pi\mid V=0) \ge \frac{2}{c+1}\cdot \I(X'_i;\Pi'). \label{eqn:3}
\end{equation}

Combining equations (\ref{eqn:1}), (\ref{eqn:2}) and (\ref{eqn:3}), we obtain the desired inequality. 

\end{proof}

%Combining Lemma~\ref{lem:mutual-info-hellinger} with Theorem 7 of~\cite{Hellinger} (restated as Theorem~\ref{thm:hellinger-sum}), we easily get the following theorem:




%\begin{proof}[Proof of Theorem~\ref{thm:main-asymmetric}]
%	First by Lemma~\ref{lem:mutual-info-additivity}, we can decompose $\I(X;\Pi)$ by 
%		$$ \I(X;\Pi\mid V=0)\ge \sum_{i=1}^m \I(X_i;\Pi\mid V=0) $$
%	Then invoking Lemma~\ref{lem:mutual-info-hellinger}, we can lower bound $ \I(X_i;\Pi)$ by the hellinger distance between $\Pi_{\bs{e_i}}$ and $\Pi_{\bs{0}}$. 
%		\begin{equation*}
%		\I(X_i;\Pi\mid V=0) \ge \Omega(\beta^{-1})\cdot \h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}})
%		\end{equation*}
%	Then by Theorem~\ref{thm:hellinger-sum}, we have
%	 $$\sum_{i=1}^{m} \h^2(\Pi_{\bs{e_i}}, \Pi_{\bs{0}}) \ge \h^2(\Pi_{\bs{0}}, \Pi_{\bs{1}}). $$
%	 
%	 Then the desired inequality follows by combining the inequalities above. 
%\end{proof}
%\begin{corollary}
%	Under the same assumption of Theorem~\ref{thm:main}, if $V$ is uniform over $\{0,1\}$ and conditioned on $V=v$, $X_1,\dots,X_m$  are generated from $\mu_v^m$, then the markov chain $V, (X_1,\dots,X_m),$$ \Pi(X_1,\dots,X_m)$ satisfies the multi-player data processing inequality with the parameter $O(\beta)$: 
%	\begin{equation}
%		\I(V;\Pi)\le O(\beta)\cdot\I( X_1\dots X_m;\Pi)
%	\end{equation}
%\end{corollary}

%The following corollary follows easily by observing that distinguishing $\mu_{\bs{0}}$ and $\mu_{\bs{1}}$ requires $\TV{\Pi_{\bs{0}}-\Pi_{\bs{1}}}$ to be large and so is $\h^2(\Pi_{\bs{0}}, \Pi_{\bs{1}})$. 
%\begin{corollary}\label{cor:main}
%	Under the assumption of Theorem~\ref{thm:main}, If a protocol $\Pi$ and a (random) function $\hat{v}$ of $\Pi$ can distinguish distribution $\mu_{\bs{0}}$ and $\mu_{\bs{1}}$ with probability $3/4$,  in the sense that for any $v \in \{0,1\}$, when $X_i$ are i.i.d from distribution $\mu_v$, 
%	$$\Pr[\hat{v}(\Pi(X)) = v] \ge  3/4.$$
%	Then when $X_i$ are i.i.d from distribution $\mu_0$, we have 
%	$$\I(X;\Pi) \ge \Omega(\beta^{-1}).$$
%\end{corollary}
%
%\begin{remark}
%	A very nice feature of this corollary  is that it is prior-free in the sense that in the statement of the theorem, we don't have a prior on the hidden variable $V$. This was the main difficulty since when $V$ has a very biased prior distribution, the approach of~\cite{DBLP:journals/corr/DuchiJWZ14} seems hard to be generalized especially in the multi-round communication case. On the other hand, the condition of our theory only requires data processing inequality with $V$ having uniform Bernoulli distribution, which is the relative easy case for data processing inequality. 
%\end{remark}

